A First Look into the Structural Properties and Resilience of Blockchain Overlays

Blockchain (BC) systems are highly distributed peer-to-peer networks that offer an alternative to centralized services and promise robustness to coordinated attacks. However, the resilience and overall security of a BC system rests heavily on the structural properties of its underlying peer-to-peer overlay. Despite their success, BC overlay networks' critical design aspects, connectivity properties and network-layer inter-dependencies are still poorly understood. In this work, we set out to fill this gap and study the most important overlay network structural properties and robustness to targeted attacks of seven distinct BC networks. In particular, we probe and crawl these BC networks every two hours to gather information about all their available peers, over a duration of 28 days. We analyze 335 network snapshots per BC network, for a total of 2345 snapshots. We construct, at frequent intervals, connectivity graphs for each BC network, consisting of all potential connections between peers. We analyze the structural graph properties of these networks and compare them across the seven BC networks. We also study how these properties associate with the resilience of each network to partitioning attacks, i.e., when peers are selected, attacked and taken offline, using different selection strategies driven by the aforementioned structural properties. In fact, we show that by targeting fewer than 10 highly-connected peers, major BCs such as Bitcoin can be partitioned into disjoint, i.e., disconnected, components. Finally, we uncover a hidden interconnection between different BC networks, where certain peers participate in more than one BC network, which has serious implications for the robustness of the overall BC network ecosystem.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> p_tbl_full_basic_info.tex <==
\begin{table}[]
\caption{Bitcoin: average metrics}
\label{tab:btc-basic}
\begin{tabular}{lr}
\midrule
Nodes &37131\\ 
Edges &2587040\\ 
Zero Deg Nodes &0.0\\ 
Zero InDeg Nodes &6\\ 
Zero OutDeg Nodes &33533\\ 
NonZero In-Out Deg Nodes &3592\\ 
Unique directed edges &2587040\\ 
Unique undirected edges &2504867\\ 
Self Edges &612\\ 
Bi-Directional Edges &164958\\ 
Frac. of closed triads &0.031\\
Connected component size &0.99\\
Strong conn. comp. size &0.08\\
Approx. full diameter &4\\ 
90\% effective diameter &2\\
\end{tabular}
\end{table}



\begin{table}[]
\caption{BitcoinCash: average metrics}
\label{tab:bch-basic}
\begin{tabular}{lr}
\midrule
Nodes &23013\\
Edges &169020\\
Zero Deg Nodes &0\\
Zero InDeg Nodes &0\\
Zero OutDeg Nodes &22060\\
NonZero In-Out Deg Nodes &952\\
Unique directed edges &169020\\
Unique undirected edges &164730\\
Self Edges &431\\
Bi-Directional Edges &9012\\
Frac. of closed triads &0.01\\
Connected component size &0.99\\
Strong conn. comp. size &0.04\\
Approx. full diameter &4\\
90\% effective diameter &2\\
\hline
\end{tabular}
\end{table}


\begin{table}[]
\caption{DASH: average metrics}
\label{tab:dash-basic}
\begin{tabular}{lr}
\midrule
Nodes &8485\\  
Edges &7312276\\  
Zero Deg Nodes &0\\ 
Zero InDeg Nodes &10\\
Zero OutDeg Nodes &1498\\  
NonZero In-Out Deg Nodes &6975\\  
Unique directed edges &7312276\\  
Unique undirected edges &6724697\\  
Self Edges &576\\ 
Bi-Directional Edges &1175733\\ 
Frac. of closed triads &0.16\\
Connected component size &1.0\\
Strong conn. comp. size &0.82\\
Approx. full diameter &4\\ 
90\% effective diameter &1\\
\end{tabular}
\end{table}

\begin{table}[]
\caption{Dogecoin: average metrics}
\label{tab:doge-basic}
\begin{tabular}{lr}
\midrule
Nodes &1214\\  
Edges &116376\\  
Zero Deg Nodes &0\\
Zero InDeg Nodes &9\\
Zero OutDeg Nodes &881\\  
NonZero In-Out Deg Nodes &324\\ 
Unique directed edges &116376\\ 
Unique undirected edges &93785\\ 
Self Edges &85\\ 
Bi-Directional Edges &45267\\  
Frac. of closed triads &0.28\\
Connected component size &1.0\\
Strong conn. comp. size &0.27\\
Approx. full diameter &3\\ 
90\% effective diameter &2\\ 
\end{tabular}
\end{table}

\begin{table}[]
\caption{Ethereum: average metrics}
\label{tab:eth-basic}
\begin{tabular}{lr}
\midrule
Nodes &11887\\ 
Edges &59297\\ 
Zero Deg Nodes &0\\
Zero InDeg Nodes &16\\
Zero OutDeg Nodes &11120\\ 
NonZero In-Out Deg Nodes &750\\ 
Unique directed edges &59297\\ 
Unique undirected edges &59180\\ 
Self Edges &9\\
Bi-Directional Edges &243\\ 
Frac. of closed triads &0.002\\
Connected component size &0.99\\
Strong conn. comp. size &0.04\\
Approx. full diameter &6\\ 
90\% effective diameter &4\\
\end{tabular}
\end{table}

\begin{table}[]
\caption{Litecoin: average metrics}
\label{tab:ltc-basic}
\begin{tabular}{lr}
\midrule
Nodes &8205\\ 
Edges &741502\\ 
Zero Deg Nodes &0\\
Zero InDeg Nodes &0\\
Zero OutDeg Nodes &7052\\
NonZero In-Out Deg Nodes &1152\\ 
Unique directed edges &741502\\ 
Unique undirected edges &707683\\ 
Self Edges &101\\
Bi-Directional Edges &67738\\ 
Frac. of closed triads &0.07\\
Connected component size &1.0 \\
Strong conn. comp. size &0.16\\
Approx. full diameter &4\\ 
90\% effective diameter &2\\
\end{tabular}
\end{table}


\begin{table}[]
\caption{ZCash: average metrics}
\label{tab:zec-basic}
\begin{tabular}{lr}
\midrule
Nodes &1457 \\
Edges &106890 \\
Zero Deg Nodes &0 \\
Zero InDeg Nodes &0 \\
Zero OutDeg Nodes &1218 \\
NonZero In-Out Deg Nodes &239 \\
Unique directed edges &106890 \\
Unique undirected edges &82399 \\
Self Edges &131 \\
Bi-Directional Edges &49115 \\
Frac. of closed triads &0.31\\
Connected component size &1.0\\
Strong conn. comp. size &0.17\\
Approx. full diameter &4 \\
90\% effective diameter &2.2 \\
\end{tabular}
\end{table}

==> tmp_related.tex <==
\section{Related Work}
\label{sec:related}
\mysubsubsection{BC Topology Inference.}
Miller \etal~\cite{coinscope} were the first to attempt to infer Bitcoin's public network topology.
They discovered links between nodes by leveraging the timestamps included in \texttt{ADDR} messages.
% Before this work, peers responded to \texttt{GETADDR} messages, including a timestamp for each IP address.
% The timestamp’s role was to ensure that terminated nodes were not propagated in the network anymore.
% The nodes regularly refreshed timestamps. Thus, by issuing \texttt{GETADDR} messages to all reachable nodes in the network and analyzing the timestamps, Miller \etal managed to obtain a map of connections.
In their work, as in ours, they also find indications that the Bitcoin network is not purely random.
% Unfortunately, this method cannot be used anymore.
% Bitcoin's core developers decided to hide this information in release 0.10.1~\cite{millerban}.  
% Their reasoning was to discourage topology inference to enhance security from potential adversaries.
Grundmann \etal~\cite{GrundmannNH18} explored two mechanisms for Bitcoin topology inference.
Their first approach exploits the accumulation of multiple transactions before their announcement to other peers but results in a low inference quality. Their second approach exploits the fact that clients drop double--spending transactions. Using this information, they accurately infer a peer's connections. 
However, this method was not intended to perform full network topology inference due to high cost: with current transaction fees, inferring the connections of a single peer would cost around \$78~\cite{bitcoinfees}.
Both methods of~\cite{GrundmannNH18} require maintaining connections to all reachable peers and crafting distinguishable transactions, one for each reachable peer. Due to ethical reasons, their validation was performed against Bitcoin's testnet.

Delgado-Segura \etal~\cite{txprobe} devised a different method to infer Bitcoin's network topology, using orphaned transactions. Their method relies on subtleties of Bitcoin's transaction propagation behavior.
It involves fabricating double--spending transaction pairs and sending them to a part of the network.
Since their method could interfere with ordinary transactions, they have only performed measurements in Bitcoin's testnet. Their results also indicate that Bitcoin's testnet does not resemble a random graph.
Using this method with current Bitcoin prices and 11,000 reachable Bitcoin nodes would require more than \$5,700 in transaction fees and more than 12 hours to cover the whole network~\cite{bitcoinfees}.

Neudecker \etal~\cite{btctiminganalysis} performed a timing analysis of the propagation of transactions to infer the network topology. In contrast to Miller \etal, Neudecker \etal~use transaction propagation delays, as observed by a highly connected monitor, to infer topology. By observing timestamps of reception of certain transactions and utilizing a propagation delay model, they infer the path of transaction and, thereby, connections between peers.
This approach requires the monitoring node to actively create transactions if it cannot determine the transaction originator.
Furthermore, changes made to the Bitcoin Core reference client, render this method impractical~\cite{bitcoin_pr7125}.
%This PR changed the forwarding behavior for transactions from trickling to random delays per neighbor. The randomization introduced a high uncertainty for timing analysis using transactions.

By exploiting block relay mechanisms, Daniel \etal~\cite{mapz} presented a passive method to infer connections of mining nodes and their direct neighbors in the ZCash network. Biryukov \etal~\cite{DBLP:conf/ccs/BiryukovKP14} focused on deanonymizing Bitcoin users by suggesting a method for topology discovery by sending fake marker IP addresses to remote peers. Neudecker and Hartenstein~\cite{NeudeckerH19} surveyed the network layer of permissionless BCs, simulated a passive method to infer the network topology with substantial accuracy, and emphasized how network topology hiding is an intermediate security requirement. Decker \etal~\cite{Decker2013} measured the rate of information propagation throughout the network and showed, among other findings, that delays in block propagation are highly correlated to chain forks.
Finally, work from Dotan \etal~\cite{pingoletSOK} presents a structured overview of BC P2P overlay networks.
Their work highlights differences and commonalities with traditional networks and identifies open research challenges in network design for decentralized distributed systems.

% \mysubsubsection{Node Eclipsing and Partitioning Attacks.}
% Heilman and Kendler presented an eclipse attack on Bitcoin’s P2P network~\cite{eclipseattack}. 
% They demonstrate how an adversary controlling a large number of IP addresses can monopolize all connections to and from a victim node and exploit it to mount attacks on Bitcoin's mining and consensus. A similar attack has been demonstrated by Marcus \etal~\cite{etheclipse_gen}. It is applicable to the Ethereum BC, and was further optimized in~\cite{etheclipse}.
% Saad \etal~\cite{Saad19, Saad2019} explore various partitioning attacks of the Bitcoin network. Neudecker~\cite{NeudeckerAH15} also explores the feasibility of partitioning attacks through a simulated analysis.
% Partitioning of the Bitcoin network through BGP hijacks was studied by Apostolaki \etal~\cite{Apostolaki2017}. 
% Such works rely on the spatial concentration of nodes within an AS or an ISP, which makes them vulnerable to routing attacks. More recently, Tran \etal~\cite{Tran20erebus} proposed a stealthier version of a partitioning attack.

%\nk{At the end of the related work, clearly state in a short paragraph what we do above and beyond this related work.}
%\mysubsubsection{Summary.}
\rc{More clarity is needed in how certain previously applied methods are not applicable anymore. For example, more explanation is needed on what changes in the Bitcoin Core client render Neudecker's methods not applicable. Overall, the dismissal of previous methods seems cursory at times to the reader (although it might well not be), so some more sound justification of the need for a new method would help.}
Despite previous efforts, very little is known regarding the structure and topological properties of BC overlay networks.
Instead, past studies focused on methods for inferring the well--hidden topology of Bitcoin, either against the whole network or a specific peer.
With the exception of~\cite{coinscope}, these studies were validated against the Bitcoin testnet~\cite{txprobe}, or against selected nodes~\cite{btctiminganalysis, GrundmannNH18}.

Topology inference in BC networks remains an unsolved problem. 
%\ms{do we solve it here? If yes, state so explicitly and explain how/why} 
Most suggested methods are either not applicable anymore due to changes in the reference clients, infeasible due to transaction fees, or impractical to run against multiple BC networks since they require maintaining connections to a high number of peers.
Furthermore, Bitcoin core developers are constantly updating protocol subtleties to prevent leakage of information that would ease topology inference.

%\mysubsubsection{Contributions.}
To the best of our knowledge, this is the first study that focuses on various BC networks'  structural properties.
As we show in Sec.~\ref{sec:methodology-assessment}, we circumvent the challenges of topology inference and build a simple network monitor that can probe seven different BC networks in parallel.
Our implementation does not require high connectivity in each network and is free of transaction processing costs, allowing for greater scalability.
Similar to~\cite{coinscope}, our work does not interfere with transactions and only uses information made available by the network peers. % (Sec.~\ref{sec:methodology}).
We are the first to study the crawled BC networks in--depth for their network characteristics and properties.
Furthermore, we investigate the resilience of these networks against random and targeted attacks.



==> u_resilience.tex <==
\section{Topology Robustness}

% \subsection{Algebraic connectivity}
% From wikipedia:
% The algebraic connectivity (also known as Fiedler value or Fiedler eigenvalue) of a graph G is the second-smallest eigenvalue (counting multiple eigenvalues separately) of the Laplacian matrix of G. This eigenvalue is greater than 0 if and only if G is a connected graph. This is a corollary to the fact that the number of times 0 appears as an eigenvalue in the Laplacian is the number of connected components in the graph. The magnitude of this value reflects how well connected the overall graph is. It has been used in analysing the robustness and synchronizability of networks.
% Fiedler's paper~\cite{fiedler73algebraic}
% The algebraic connectivity of a graph is defined as the second smallest eigenvalue
% of its Laplacian matrix $L$, $\lambda_{2}(L)$ and is a lower bound on node/edge connectivity~\cite{fiedler73algebraic}.


% \begin{table}[]
% \caption{Algebraic Connectivity}
% \label{tab:fiedler}
% \begin{tabular}{|l|r|c|c|ll|}
% \hline
% \multirow{2}{*}{Network} & \multicolumn{2}{r|}{\begin{tabular}[c]{@{}l@{}}Edges \\ Removed\end{tabular}} & \multirow{2}{*}{Split} & \multirow{2}{*}{Cut-ratio} &\\
%  & \# & \%&&&\\
%  \hline
% Bitcoin     & 5545          &0.1          & 9964/43949  &0.23  &  \\
% \hline
% BitcoinCash & 10603         &6.5            & 11895/11367 &1.05  &  \\
% \hline
% DASH        & 1451          &0.02            & 46/8556     &0.005  &  \\
% \hline
% Dogecoin    & 581           &0.44            & 11/1069     &0.01  &  \\
% \hline
% Ethereum    & 2220          &2.72            & 436/15345   &0.03  &  \\
% \hline
% Litecoin    & 544           &0.08            & 37/6576     &0.006  &  \\
% \hline
% ZCash       & 363           &0.33            & 258/1231    &0.3  & \\
% \hline
% \end{tabular}
% \end{table}

% %%The fiedler vectors (shown in Table \ref{tab:fiedler})
% %%were computed using the \texttt{fiedler\_vector} method of NetworkX package.
% The Fiedler vector yields a lower bound on the optimal cost
% of ratio-cut partition which bisects the graph into two communities, based on the sign of the corresponding vector entry. 
% Division into a larger number of communities can be achieved by repeated bisection or by using multiple eigenvectors corresponding to the smallest eigenvalues.
% Computing the Fiedler vector in all snapshots we have collected was prohibitive. Table \ref{tab:fiedler} shows the number of edges removed and the cut-ratio of a selected snapshot for each blockchain.
% Most cuts are heavily unbalanced with the exception of BitcoinCash which
% almost has a perfect cut (albeit, by removing a high fraction of edges).
% Bitcoin has a one-to-five cut by removing a 0.1\% of the edges.


\subsection{Node Percolation}
It is known that scale-free networks are highly resilient to random failures. 
On the other hand, they are less robust on targeted attacks. 
In this section we perform a similar assessment on the derived graphs.
Since the networks of interest do not have the scale-free property we are interested in both their random failure and attack robustness.
We do not study targeted link removals since their removal is usually less effective, while the removal of a node simultaneously cut all its adjacent links.
We follow a static technique in the sense that each node is given a priority of removal once based on some criterion. After a node removal priorities are not recalculated. The nodes are then removed from the network one by one following the given priority. After each node removal we re-calculate the size of the largest (weakly) connected component and the approximate diameter of the resulting graph. The criteria used in this study are the betweenness centrality of a node and its node-index (cf node index explanation).
We performed the procedure described above for all snapshots we have constructed. Due to high number of graphs collected, we stop execution after removing 12\% of the nodes from each snapshot.
In Figure \ref{fig:percolation-low} 
we report our findings in number of nodes removed 
and in Figure \ref{fig:percolation-high} in percentage of nodes removed.

\begin{figure}
\centering
    \subfloat[\centering Bitcoin]{{\includegraphics[width=5cm]{figures/percolation/Bitcoin-perc11-evo.png} }}%
    \subfloat[\centering BitcoinCash]{{\includegraphics[width=5cm]{figures/percolation/BitcoinCash-perc11-evo.png} }}%
    \subfloat[\centering DASH]{{\includegraphics[width=5cm]{figures/percolation/DASH-perc11-evo.png} }}%
    \quad
    \subfloat[\centering Dogecoin]{{\includegraphics[width=5cm]{figures/percolation/Dogecoin-perc11-evo.png} }}%
    \subfloat[\centering Ethereum]{{\includegraphics[width=5cm]{figures/percolation/Ethereum-perc11-evo.png} }}%
    \subfloat[\centering Litecoin]{{\includegraphics[width=5cm]{figures/percolation/Litecoin-perc11-evo.png} }}%
    \quad
    \subfloat[\centering ZCash]{{\includegraphics[width=5cm]{figures/percolation/ZCash-perc11-evo.png} }}%
    \caption{Evolution of the largest connected component and the approximate diameter while removing nodes one by one.
    Lines correspond to the computed average over all snapshots.
    The area between the minimum and maximum values is shaded.
    Red corresponds to the betweenness strategy; blue to the node-index.
    X-axis represents the number of nodes removed.}%
\label{fig:percolation-low}%
\end{figure}


\begin{figure}[htbp]
  \centering
  \subfloat[\centering Bitcoin]
  {{\includesvg[width=5cm]{figures/percolation/Bitcoin-evo60Qs.svg}}}%
  \subfloat[\centering BitcoinCash]
  {{\includesvg[width=5cm]{figures/percolation/BitcoinCash-evo60Qs.svg}}}%
  \subfloat[\centering DASH]
  {{\includesvg[width=5cm]{figures/percolation/DASH-evo60Qs.svg}}}%
  \quad
  \subfloat[\centering Dogecoin]
  {{\includesvg[width=5cm]{figures/percolation/Dogecoin-evo60Qs.svg}}}%
  \subfloat[\centering Ethereum]
  {{\includesvg[width=5cm]{figures/percolation/Ethereum-evo60Qs.svg}}}%
  \subfloat[\centering Litecoin]
  {{\includesvg[width=5cm]{figures/percolation/Litecoin-evo60Qs.svg}}}%
  \qquad
  \subfloat[\centering ZCash]
  {{\includesvg[width=5cm]{figures/percolation/ZCash-evo60Qs.svg}}}%
  \caption{Evolution of the largest connected component and the approximate diameter when the network in under targeted attack.
    Lines correspond to the median value across all snapshots.
    The area between the 1st and 3rd quantile is shaded.
    Red corresponds to the betweenness strategy,
    blue to the node-index, and green to random.
    X-axis reports the percentage of nodes removed.}%
\label{fig:percolation-high}%
\end{figure}


Studying the evolution of the relative size of the largest connected component, we observer that Bitcoin and BitcoinCash networks are very sensitive to targeted node removals. It is worth mentioning that, in average, removal of the top five nodes, reduces the largest connected component to 40\% of its initial size. 
This finding is particularly worrying indicating that these networks could be prone to partitioning attacks. 
ZCash follows a similar behavior, although less severe. 
By contrast Ethereum seems to have the most robust topology, followed by DASH, Litecoin and Dogecoin. These networks exhibit a higher level of robustness even after removing a significant portion of nodes (>10\%).


Findings - in simple words:
Bitcon: 
The removal of the top 5 nodes, (ranked in accordance to betweenness centrality) 
reduces the size of the largest connected component to 40\% of the initial network.
For some specific snapshots the size drops further to 20\%.
If we continue removing nodes we couldn't identify a dramatic change to the network's connectivity in the average case.
Nevertheless, in some cases 90\% of the nodes would get disconnected by removing 2\% of the nodes.
%%I.e by removing 720 nodes the network would disconnect 90\% of the nodes
Ta idia kai xeirotera me to bitcoincash opou parateireite kai ayjisi sti diametro to diktyou.

Dogecoin and DASH exhibit an extreme robustness, which can be tracked back to their structural properties (high density, large strongly connected component, high average clustering) mentioned in the previous section.
Ethereum shows a good robustness as well, although less than DASH and Dogecoin.
Interestingly, our "best" effort at disconnecting the network was when using 
our alternative strategy (by ranking on the node \textit{index value} (see eqn \ref{nodeindex:eqn}).

\subsubsection{Targeting Overlapping Nodes}
Perhaps a more interesting finding is when considering common nodes.
Merely by the fact these nodes participate in more than one blockchains draws our attention to them.
By removing those nodes first, at the same time from all graphs, we obtain the following results in fig. \ref{fig:resilience_vlops}:

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/overlaps/vlapsConCompSzevolution.png}
    \caption{Relative change of the size of the largest connected component while removing common nodes.}
    \Description{resilience_rem_comm}
    \label{fig:resilience_vlops}
\end{figure}






==> u_structural.tex <==
\section{Structural properties}
\color{blue}
NK: what research questions are we answering in each result section ?
state them at the begining of each.

Here we want to answer what are the network characteristics
of blockchain overlay networks. Do they share common properties among them, or with other known networks?
\color{black}

Table \ref{tab:basic-all} summarizes the basic information of the derived graphs. 
All networks are connected and have low diameters. Most networks have a diameter equal to 4. Exceptions are Ethereum having a diameter of 6 hops and Dogecoin having the smallest diameter equal to 3 hops.
Bitcoin is the largest network having more than 50k nodes. BitcoinCash and Ethereum follow, having sizes close to 20k and 10k nodes.
DASH and Litecoin have similar sizes around 8k nodes. The two smallest networks are ZCash and Dogecoin with less than 2k nodes.
Moreover, we observe that DASH is by far the most dense network and is almost fully connected, having a strongly connected component close to 0.8. Despite DASH, the larger networks have a smaller strongly connected component compared to Dogecoin and ZCash.
\input{p_tbl_basic_info}

\color{red}
\subsection{Degree Distribution}
%%Barabasi:
A key property of each node is its degree, representing the number of links it has to other nodes.
The degree distribution, $pk $, provides the probability that a randomly selected node in the network has degree $k$.
The degree distribution has assumed a central role in network theory following the discovery of scale-free networks [8].
Additionally, the precise functional form of $pk$ determines many network phenomena, including network robustness and efficiency in 
information dissemination.
A random network has a binomial distribution, 
but in real systems we have more highly connected nodes than the random network model could account for.
%%
%%Bitcoin - indeg : std -> 196.4947583713169 <k>^1/2 --> 9.838456125655274
%%BitcoinCash - indeg : std -> 21.965096171131055 <k>^1/2 --> 2.8886845526618616
%%DASH - indeg : std -> 560.2157757639978 <k>^1/2 --> 29.380480238579946
%%Dogecoin - indeg : std -> 88.48671326055201 <k>^1/2 --> 9.8471616437873
%%Ethereum - indeg : std -> 7.90042081938626 <k>^1/2 --> 2.4462446466646366
%%Litecoin - indeg : std -> 89.8067595758737 <k>^1/2 --> 9.553751712262219
%%ZCash - indeg : std -> 87.65685492225971 <k>^1/2 --> 8.621528259193932
%%Bitcoin - outdeg : std -> 388.7353924992127 <k>^1/2 --> 9.838456125655274
%%BitcoinCash - outdeg : std -> 148.0329655953075 <k>^1/2 --> 2.8886845526618616
%%DASH - outdeg : std -> 879.770485410528 <k>^1/2 --> 29.380480238579946
%%Dogecoin - outdeg : std -> 173.6900271842186 <k>^1/2 --> 9.8471616437873
%%Ethereum - outdeg : std -> 22.82551968370399 <k>^1/2 --> 2.4462446466646366
%%Litecoin - outdeg : std -> 271.39072151539307 <k>^1/2 --> 9.553751712262219
%%ZCash - outdeg : std -> 173.5031197929831 <k>^1/2 --> 8.621528259193932
A scale-free network is a network whose degree distribution follows a power law, $ P(k) \sim \ k^{-\gamma}$ .
Many researches show that many real-world networks like the Internet topology of ASes, the Web, and social networks, follow a power-low in their degree distributions. 
The same has been stated for the Bitcoin overlay network [cite refs]. 
Others mention that blockchain overlay networks (Bitcoin in particular) form random graphs. [cite  Information propagation , SOK]
By studying the complementary CDF of degree distributions shown in Figure \ref{fig:ccdf-deg-dist}, a clear power-law trend is not evident.
Nevertheless, we observe a high standard deviation in the degree distributions, one of the characteristics of scale-free networks.
%%In most distributions we see a peak forming near the tail, resembling to a normal distribution. Based on the metrics we study later in this section, we also observe that the networks have different characteristics from random generated graphs.
\begin{figure}
\centering
    \subfloat[\centering In-degree]{
    {\includegraphics[width=0.4\textwidth]{figures/degree__dists/indeg-all.png}}}%
    \subfloat[\centering Out-degree]{
    {\includegraphics[width=0.4\textwidth]{figures/degree__dists/outdeg-all.png}}}%
    \caption{Degree distributions}%
\label{fig:ccdf-deg-dist}%
\end{figure}
\begin{figure}
\centering
    \subfloat[\centering Bitcoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_btc.png}}}%
    \subfloat[\centering BitcoinCash]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_bch.png}}}%
    \qquad
    \subfloat[\centering DASH]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_dash.png}}}%
    \subfloat[\centering Dogecoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_doge.png}}}%
    \qquad
    \subfloat[\centering Ethereum]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_eth.png}}}%
    \subfloat[\centering Litecoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_ltc.png}}}%
    \qquad
    \subfloat[\centering ZCash]{{\includegraphics[width=3.8cm]{figures/degree__dists/in_zec.png}}}%
    \caption{In-degree distributions}%
\label{fig:deg-dist}%
\end{figure}
\subsection{Clustering Coefficient}
The local clustering coefficient $C_i$ measures the density of links in node $i$’s immediate neighborhood: $C_i = 0 $means that there are no links between $i$’s neighbors; $C_i = 1 $implies that each of the $i$’s neighbors link to each other.
In a random network the local clustering coefficient is independent of the node’s degree and average clustering coefficient \textit{<C>} depends on the system size as $<k>/N$ \cite{barabasi2016network}. 
In contrast, measurements indicate that for real networks the clustering coefficient decreases with the node's degree and is largely independent of the system size.
The local clustering coefficient $C_{rand}$ in a random network 
is calculated as the average degree $<k>$ over the total number of nodes $N$,
$C_{rand} = \frac{<k>}{N}$\footnote{Subsequently the average clustering of the network is the same.}
According to the same source the average degree of a network is equal to $\frac{2L}{N}$, where $L$ 
is the number of links and $N$ is the number of nodes.
The average clustering coefficient of a real network is expected to be much higher than a random graph. 
Figure \ref{fig:cc-all}(a) compares the average clustering coefficient of the networks of interest with the prediction for random networks of same size. The markers and their colors correspond to the networks of Table \ref{tab:basic-all}.
Barabasi \cite{barabasi2016network} reports that
\textit{In summary, we find that the random network model does not capture the clustering of real networks. Instead real networks have a much higher clustering coefficient than expected for a random network of similar N and L.}

Surprisingly, we observer some irregularities from known trends. 
Some high degree nodes in Bitcoin, Ethereum and ZCash have very high clustering coefficients; something unusual in real netowrks.
DASH has a different behaviour: all nodes seem to have very similar clustering coefficients, independent from the node's degree; an exception to this empirical rule for real networks.

\begin{figure}[htbp]
  \centering
  \subfloat[\centering All Networks]
  {{\includegraphics[width=0.22\linewidth]{figures/clustering/all_nets_ccVsdegree.png}}}%
  \subfloat[\centering Bitcoin]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_Bitcoin.svg}}}%
  \subfloat[\centering BitcoinCash]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_BitcoinCash.svg}}}%
  \subfloat[\centering DASH]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_DASH.svg}}}%
  \quad
  \subfloat[\centering Dogecoin]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_Dogecoin.svg}}}%
  \subfloat[\centering Ethereum]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_Ethereum.svg}}}%
  \subfloat[\centering Litecoin]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_Litecoin.svg}}}%
  \subfloat[\centering ZCash]
  {{\includesvg[width=0.22\linewidth]{figures/clustering/cc_ZCash.svg}}}%
  \quad
  \caption{Clustering Coefficient. \\
    (a) $\frac{<C>}{<k>}$ vs network size.
    Markers correspond to the networks of Table \ref{tab:basic-all}. 
    Lines correspond to the prediction of the clustering coefficient for random networks.
    Similar to other known networks the average clustering appears to be independent of N.
    \\
    (b)-(h) The dependence of the local clustering coefficient, $C(k)$, on the node’s degree for each network. $C(k)$ is measured by averaging the local clustering coefficient of all nodes with the same degree $k$. 
    Horizontal lines corresponds to the average clustering coefficient.
    }
    \Description{Comparison of the average clustering coefficient of blockchain networks with the prediction for random networks.}
\label{fig:cc-all}%
\end{figure}


\subsection{Betweeness Centrality and PageRank}
\subsection{Discussion}

\textit{Discuss small worldness, comparison to random graphs and other known networks (Internet AS topology, the Web, social networks.}
introduce the nodeindex we devised to summarize all metrics.
\paragraph{Small-World property}
%%Barabasi:
The small world phenomenon states that if you choose any two individuals 
nodes of a small-world graph, the distance between them will be relatively short;
orders of magnitude smaller than the size of the network.
According to \cite{barabasi2016network}, the small world property is typically defined by:
$  <d> \approx \frac{lnN}{ln<k>}   $, 
where $<d>$ is the average distance\footnote{Or the average shortest path length.} and $<k>$ is the average degree of the network.
Based on the collected data, we calculated the average distance for each snapshot and calculated the 
value of $\frac{lnN}{ln<k>}$.
Table \ref{tab:smallworld} reports the median difference (accross all snapshots) of the two values for each network. 
By considering the sizes reported in Table \ref{tab:basic-all},
we can observe that all networks of interest adhere to the small-world property.
\begin{table}
\caption{Small World property. 
Reporting the median difference (across all snapshots) between $<d>$ and $ \frac{lnN}{ln<k>}  $}
\label{tab:smallworld}
\begin{tabular}{ |l|r|r| } 
 \hline
 Netowrk & $<d>$ - $\frac{lnN}{ln<k>}$ \\
 \hline
 Bitcoin     &0.15 \\
 BitcoinCash &-2.29 \\
 DASH        &0.57 \\
 Dogecoin    &0.12 \\
 Ethereum    &-2.55 \\
 Litecoin    &0.07 \\
 ZCash       &-0.08 \\
 \hline
\end{tabular}
\end{table}

\subsection{Robustness}
Here we study the robustness of each snapshot against random failures and targeted attacks.
We study attacks based on the following metrics: 
Betweeness centrality, node out-degree, and node-index (cf. \ref{nodeindex:eqn}.

We rank nodes in descending order of each strategy. 
For each snapshot we remove nodes from the graph according to the defined strategy ordering.
Figure \ref{fig:percolation-high} shows the aggregated results against each network. 
The line plot represents the median accross all snapshots 
The interquantile range is represented by the shaded areas.

\color{black}

\subsection{Degree Distributions}



\subsection{Small-world property}


\subsection{Clustering Coefficient}









\subsection{Degree Correlation and Assortativity}
In a random network one does not expect to find a hub, a node with very high degree. In real networks however this is something rather common.
In some networks hubs tend to link to other hubs, 
while in others hubs tend to link to low degree nodes; what is known as a hub-and-spoke pattern.
In general a network displays degree correlations if the number of links between the high and low-degree nodes is systematically different from what is expected by chance. 

Assortativity, or assortative mixing is a preference for a network's nodes to attach to others that are similar in some way. Though the specific measure of similarity may vary, network theorists often examine assortativity in terms of a node's degree. The addition of this characteristic to network models more closely approximates the behaviors of many real world networks.

Correlations between nodes of similar degree are often found in the mixing patterns of many observable networks. For instance, in social networks, nodes tend to be connected with other nodes with similar degree values. This tendency is referred to as assortative mixing, or assortativity. On the other hand, technological and biological networks typically show disassortative mixing, or disassortativity, as high degree nodes tend to attach to low degree nodes.

Assortativity is the preference of a network's nodes to attach to others 
with similar degree. 
The assortativity coefficient, $\rho$, is the Pearson correlation coefficient of degree between pairs of linked nodes. 
It lies in the range $ -1 \leq \rho \leq 1$. 
A network is said to be assortative ($\rho$ tends to 1) when high-degree nodes tend to link to each other and avoid linking to small-degree nodes, while low-degree nodes tend to connect to other small-degree nodes.
A network is said to be disassortative ($\rho$ tends to -1) when the opposite happens.
A random network with $\rho$ close to zero is characterized as neutral.

observing the correlation of in and out degrees for each network (cf. Figure \ref{fig:deg-corr-dist}) we find some characteristics similar to the Web and online social networks. In the Web, the number of pages that have high out-degree is not the same as the number of pages that have high in-degree \cite{webstruct}. On the other hand, in social networks, nodes with very high out-degree also tend to have very high in-degree \cite{socialnetsanalysis}. 
In Bitcoin, BitcoinCash, and DASH most nodes have similar out-degrees and in-degrees, while a smaller fraction of nodes have higher in-degrees than out-degrees. Additionally, some nodes have significantly higher out-degrees than in-degrees. This characteristic is similar to the Web structure. Moreover, in Dogecoin, Litecoin, and ZCash networks, nodes have a high correlation between in and out-degrees, a characteristic similar to online social networks. A possible explanation of this result is the size of these netwrorks; these are the smallest networks of our study In Ethereum, due to its distinguished discovery mechanism, the vast majority of nodes have a very high out over in-degree ratio. 

\begin{figure}
\centering
    \subfloat[\centering Bitcoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/btc.png}}}%
    \subfloat[\centering BitcoinCash]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/bch.png}}}%
    \qquad
    \subfloat[\centering DASH]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/dash.png}}}%
    \subfloat[\centering Dogecoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/doge.png}}}%
    \qquad
    \subfloat[\centering Ethereum]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/eth.png}}}%
    \subfloat[\centering Litecoin]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/ltc.png}}}%
    \qquad
    \subfloat[\centering ZCash]{{\includegraphics[width=3.8cm]{figures/degree__dists/degree_correlations/zec.png}}}%
    \caption{Degree Correlation Distribution ($Out/In$ ratio)}%
\label{fig:deg-corr-dist}%
\end{figure}


\subsection{Reciprocity}
\paragraph{Reciprocity} is a measure of likelihood of vertices in a directed graph to be mutually linked.
It has been shown to be critical in modeling and classification of directed networks. Table \ref{tab:compare-all} lists the median reciprocity accross all snapshots for each network.



\paragraph{Summary of network characteristics}
We investigated whether blockchain overlay networks have properties that
one often finds in other known networks. 
We found that they don't follow power-law degree distributions 
and we are therefore reluctant to characterize them as scale-free. 
They are also dissimilar to random networks.
They have clustering distributions that are common to real networks, 
and differ from random networks with similar size and average degree (with the exception of DASH).
All networks satisfy the small world property. 
Like most technological networks they have negative assortativity
and reciprocity varies; 
DASH has a strange clustering vs degree distribution; most probably due to its temporal characteristics (cf. section \ref{sec:temporal}: very low churn, most nodes are always online).
Their degree correlations show similar signs of known networks. 
Nevertheless, not all networks follow the same rules.
If we were to study these models in more depth new generating models are required.

Finally, we also calculated the betweenness centrality 
and page rank of each node in all snapshots.
To summarize all calculated properties in a single metric, we defined the \textit{NodeIndex} as: 

\begin{equation}
\label{nodeindex:eqn}
N_i = (InDeg_i 
            \times OutDeg_i 
            \times BC_i
            \times CC_i
            \times PR_i)^{\frac{1}{5}}
\end{equation}

%%\[\binom{n}{k} = \frac{n!}{k!(n-k)!}\]
where
$InDeg_{i}$ is the in-degree,
$OutDeg_{i}$ is the out-degree,
$BC_{i}$ is the betweeness centralilty
$CC_{i}$ is the clustering coefficient ,and
$PR_{i}$ is the page rank of node $i$.
The index is the geometric mean of each node's local graph metrics.
In-degree, out-degree, betweenness centrality and page rank are normalized using the min-max scaling method, grouped by snapshot.

Figure \ref{fig:other-dist} shows the cumulative distributions of the concatenated results per blockchain for betweeness centrality, page rank, and node index metric.
\begin{figure}
\centering
    \subfloat[\centering Betweeness]{{\includegraphics[width=0.3\linewidth]{figures/other_metrics/bc_norm-all-cdf.png}}}%
    \subfloat[\centering PageRank]{{\includegraphics[width=0.3\linewidth]{figures/other_metrics/pr_norm-all-cdf.png}}}%
    \subfloat[\centering
    NodeIndex]{{\includegraphics[width=0.3\linewidth]{figures/other_metrics/gmean-all-cdf.png}}}%
    \caption{Betweenness, Page Rank, and \textit{NodeIndex} distributions}%
\label{fig:other-dist}%
\end{figure}



\section{Temporal aspects}
\label{sec:temporal}
\color{red}
Jaccard similarity of consecutive snapshots.
Unique ip addresses discovered per blockchain
\color{black}

\begin{table}[]
\caption{Unique IPs discovered per blockchain}
\label{tab:unq-disc}
\begin{tabular}{l|r}
Network & Num. of IPs \\
\hline
  Bitcoin&      255923\\
  BitcoinCash&	74537\\
  DASH& 	    16845\\
  Dogecoin&	    11613\\ 
  Ethereum&	    44186\\
  Litecoin&	    51479\\
  ZCash&    	13122\\
  \hline
\end{tabular}
\end{table}

Since we gathered frequent snapshots of the networks of interest, we also performed a temporal analysis of the derived graphs. 
In Table \ref{tab:unq-disc} we report how many unique IP addresses were discovered 
during the crawling phase per blockchain.
We turned our focus on how often nodes appear in the collected snapshots. Results are presented below.
In Figure \ref{fig:node-jaccard}(a) we plot the cumulative distribution of the number of appearances of each node (ip address) in all captured snapshots. 
Figure \ref{fig:node-jaccard}(b) depicts the daily moving average of the Jaccard similarity index of discovered nodes in successive snapshots. 
DASH and Litecoin have a very high jacquard similarity index, meaning that nodes in these networks stay online for more time. In fact most nodes in the DASH overlay network appear to be continuously online, without frequent disconnections. Bitcoin’s jaccard similarity oscillates around 0.5 and a few thousand nodes are present in more than 200 snapshots. 
%Being the most popular blockchain, naturally attracts interest by many



\begin{figure}[h]
\subfloat[\centering Cumulative distribution of Node participation.]
{\includesvg[width=0.5\linewidth]{figures/jaccards/hist_cdf_all1.svg}}%
\subfloat[\centering Nodes' Jaccard similarity]
{\includesvg[width=0.5\linewidth]{figures/jaccards/all_jaccards_mva12annt.svg}}%
\caption{Node participation.}
\Description{Node participation.}
\label{fig:node-jaccard}
\end{figure}



\subsection{Overlaps among networks}
\label{overlaps}

Plot overlaps:
\texttt{comms-per-ts-per-chain.xls}
%%(έχουμε επίσης δεδομένα για ακμές όχι μόνο για κόμβους)


To study how often networks change we calculated the jaccard distance over the discovered nodes sets of consecutive snapshots, for each chain.

Vertical vs Horizontal overlaps.
Vertical overlaps: common addresses in different blockchains at the same timestamp.
Show the KS statistic results. 
The main key fact is that overlapping nodes stand out from the overall distribution.
As we will see in the next section 
in the case of Bitcoin and BitcoinCash are somewhat critical.

Horizontal overlaps: common addresses in the same blockchain at consecutive timestamps.
show difference in node-index distribution of horizontal overlaps vs other.
We can also show node-index distriibution of most frequent addresses overall.
The main takeaway is that these overlaps stand out by the general distribution.
(we can calculate the KS statistic for this instance as well)

\textbf{HOW ARE DISTINGUISHED FROM THE REST OF THE DISTRIBUTION - SEE NOTES ON STATISTICAL HYPOTHESIS TESTING. MENTION NORMALITY TESTS -> USAGE OF NON-PARAMETRIC TESTS - KS-TEST.
For common nodes (same timestamp): 
We performed the Shapiro test to check normality. We confirmed that the samples we have do not follow a normal distribution. 
Thus we used non-parametric tests.
}

Count overlapping nodes chains as time goes by (that's the new plot under \texttt{common} directory.)
What else ? 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/netmetrics/edge_ovlp.png}
    \caption{Distribution of edges in the blockchains we have studied.}
    \Description{edge-overlap}
    \label{fig:all-edge-ovlp}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/netmetrics/ip_ovlp.png}
    \caption{Distribution of distinct IP-addresses in the blockchains we have studied.}
    \Description{ip-overlap}
    \label{fig:all-ip-ovlp}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/common/newplot.png}
    \caption{Count of common edges in different chains. X-axis indicates the timestamp of each snapshot.}
    \Description{common-edges}
    \label{fig:common-edges}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/overlaps/comms_per_chain.pdf}
    \caption{Percentage of nodes that were found in more than one blockchain at the same timestamp. X-axis indicates the timestamp.}
    \Description{common-ip-addresses}
    \label{fig:comms_per_chain}
\end{figure}


\begin{table}[]
\caption{Average metrics. \newline
Robustness reports the critical threshold ($f_c$), at which a network's giant component shrinks to below 1\% of it's initial size.}
\label{tab:compare-all}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Network& Avg. Degree& Assortativity& Reciprocity& Clustering& Shortest Path& $f_c$ \\
\hline
 Bitcoin&92.80& -0.20& 0.06& 0.04890& 2.55& 10\%\\
 BitcoinCash&7.12& -0.64& 0.05& 0.01140& 2.82&4\%\\
 DASH&802.12& -0.06& 0.16& 0.16621& 1.93&>12\%\\
 Dogecoin&74.97& -0.13& 0.34& 0.28685& 1.77&>12\%\\
 Ethereum&4.29& -0.02& 0.00& 0.00222& 3.78&7\%\\
 Litecoin&104.04& -0.01& 0.09& 0.07345& 1.96&>12\%\\
 ZCash&56.96& -0.22& 0.47& 0.30939& 1.72&>12\%\\
\hline
\end{tabular}
\end{table}


\color{blue}
NK: At the end of each subsection in the results, please state one or two key takeaways, one sentence each. We can use those later to produce our summary of findings in the end.
\color{black}

==> u_summary.tex <==
\section{Summary - 31st August 2020.}
\subsection{Jaccard Distance Vs time}
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/all_jaccards_vs_time.png}
  \caption{Jaccard Distance of each snapshot (and its immediate previous one.) X-axis is dimensionless.}
  \Description{Jaccard distance of all snapshots.}
\end{figure}
\begin{itemize}
    \item \textit{Bitcoin:} Jaccard distance fluctuates around 0.5 with frequent drops to lower values near 0.1.
    
    \item \textit{BitcoinCash:} Higher than Bitcoin. It is usually near 0.8 with a few drops below 0.5 (at snapshots \#83, \#85, \#91 and \#94).
    
    \item \textit{DASH:} Jaccard distance is almost constant near 0.97 with very few drops that reach 0.88 but no less.
    
    \item \textit{Dogecoin:} Similar to BitcoinCash with less flustuations and higher values; near and above 0.8.
    
    \item \textit{Ethereum:} we observe three \textit{stable} periods with Jaccard distance near 0.8. The rest of the plot shows very high fluctuations between 0.0 and 1.0.
    
    \item \textit{Litecoin:} the index is very stable near 0.94 with 4 notable drops below 0.4 (from timestamp \#100 to \#138). This drop seems to be correlated with shifts to in and out degree distributions during the same period.
    
    \item \textit{ZCash:} the index oscillates near 0.7. We observe a couple of sudden drops below 0.3 which coincide with drops in Dogecoin on same timestamps.
\end{itemize}

\section{Common Edges between different blockchains}
Should change Fig. \ref{fig:overlap_cnt} to Jaccard distance.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/common/newplot.png}
  \caption{Common Edges for all pairs of blockchains per snapshot.}
  \Description{Common Edges.}
  \label{fig:overlap_cnt}
\end{figure}

\section{Graph Metrics}
Figures [\ref{fig:btc-jacc}, \ref{fig:bch-jacc}, \ref{fig:dash-jacc}, \ref{fig:doge-jacc}, \ref{fig:eth-jacc}, \ref{fig:ltc-jacc}, \ref{fig:zec-jacc}] plot the in-degree, out-degree, clustering coefficient and betweeness centrality distributions of each snapshot. Each figure plots a different blockchain. 
Line colours correspond to the Jaccard distance of the plotted snapshot with its immediately previous snapshot. 
The Jaccard distance is calculated over the set of nodes.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/Bitcoin.png}
  \caption{Distributions of graph metrics for Bitcoin. 
  Line colours correspond to Jaccard index.}
  \Description{Bitcoin Metrics.}
  \label{fig:btc-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/BitcoinCash.png}
  \caption{Distributions of graph metrics for BitcoinCash.
  Line colours correspond to Jaccard index.}
  \Description{BitcoinCash Metrics.}
  \label{fig:bch-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/DASH.png}
  \caption{Distributions of graph metrics for DASH.
  Line colours correspond to Jaccard index.}
  \Description{DASH Metrics.}
  \label{fig:dash-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/Dogecoin.png}
  \caption{Distributions of graph metrics for Dogecoin.
  Line colours correspond to Jaccard index.}
  \Description{Dogecoin Metrics.}
  \label{fig:doge-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/Ethereum.png}
  \caption{Distributions of graph metrics for Ethereum.
  Line colours correspond to Jaccard index.}
  \Description{Ethereum Metrics.}
  \label{fig:eth-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/Litecoin.png}
  \caption{Distributions of graph metrics for Litecoin.
  Line colours correspond to Jaccard index.}
  \Description{Litecoin Metrics.}
  \label{fig:ltc-jacc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/jaccards/ZCash.png}
  \caption{Distributions of graph metrics for ZCash.
  Line colours correspond to Jaccard index.}
  \Description{ZCash Metrics.}
  \label{fig:zec-jacc}
\end{figure}
\subsection{In-Degree distribution}
\begin{itemize}
    \item \textit{Bitcoin:}
    Group 1, with Jaccard distance close to 0.4:
    Nearly 40 to 60 \% of the nodes have an in-degree value of 10.
    Around 20\% of nodes have an in-degree between 10 and less than 100. 10\% have a degree between 100 and 200. The rest have a degree more than 200 but less than 1000. Only in a few distributions we have in degrees that surpass 1000.
    An other group forms with distributions having a jaccard distance near 0.2. In this case 90\% of nodes have a degree less than 10. The top 5\% has a degree of less than 200.
    
    \item \textit{BitcoinCash:}
    Most nodes ( near 80\%) have an in degree of less than 10. Few nodes have a degree up to 100 and even fewer have a degree more than 100. None of the nodes seems to have more than 200 incoming edges.
    \item \textit{DASH:}
    Around 20\% of nodes have an indegree less than 100. The next 10\% has less than 300. The majority of nodes have an in-degree between 800 and 1500. It is noteworthy that all snapshots have a jaccard distance close to 1.0 and distributions are very close one to another. 
    
    \item \textit{Dogecoin:}
    Around 20\% have an indegree of 10 or less.
    Almost 50\% of all nodes have a degree between 40 and 100.
    20\% have a degree bewteen 120 and 200. During our crawling experiment, close to the middle of the crawling period, a set of changes to the network caused a shift to the distributions of all metrics. This is better viewed in Fig \ref{fig:doge-time}. Interestingly, the jaccard index of Dogecoin  accross time, does not indicate a rearrangement of participating nodes.
    \begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/timestamps/Dogecoin.png}
    \caption{Distributions of graph metrics for Dogecoin.
    Line colours correspond to the timestamp of each snapshot.}
    \Description{Dogecoin Metrics.}
    \label{fig:doge-time}
    \end{figure}
    
    \item \textit{Ethererum:}
    Taking into consideration the regions with higher Jaccard index (near to 0.8). Most nodes (more than 75\%) have a degree less than 10. Very few nodes have a degree between 10 and 20. An extremely low percentage of nodes have a degree more than a few hundreds.
    \item \textit{Litecoin:}
    Two distinct groups of distributions stand out: the first one (having a green hue) corresponds to a lower Jaccard index, which occurred near the middle of the crawling period.
    In the second group, having a jaccard distance close to 1.0, the majority of nodes have a degree between 30 and 150. 20\% of the nodes have a degree that approaches 200.
    The first group has a similar shape but is "squeezed" towards the top; most nodes have a degree of 1. The rest of the nodes (around 20\%) have a degree near 60 and only a small fraction of them have a degree near 200.
    \item \textit{ZCash:}
    Near half of the nodes have a degree less than 10. From the remaining half, most have a degree close to 100 and the rest a degree close to 150.
    
\end{itemize}

\subsection{Out-Degree distribution}
\begin{itemize}
    \item \textit{Bitcoin:} We can observe two groups of distributions, distinguished by different jaccard indexes.
    In the group with the higher jaccard index (shown with a green hue) 90\% of nodes have a 0 degree. Most likely these are nodes included in the replies of other nodes but themselves were unreachable by our crawler. This may also indicate that most clients have peers in their memory that are stale.
    Around 10\% of the nodes have a degree between 200 and 1000.
    Only 3\% have a degree between 1000 and 2000. Very few nodes reach a degree of 10.000.
    In-degree and out-degree distributions differ.
    \item \textit{BitcoinCash:}
    More than 90\% of the nodes have zero out degree. A small fraction close to 3\% have a degree near 100.
    In-degree and out-degree distributions differ.
    \item \textit{DASH:}
    The out-degree distributions are similar to the in-degree distributions. More than half (60\%) of nodes have a degree between 200 and 1000. Around 20\% of nodes have higher degrees, up to 2000.
    \item \textit{Dogecoin:}
    Like the in degree, we can observe 2 different groups having a different jaccard index.
    65\% of nodes have 0 degree. The rest of the nodes have a degree near 200. Few nodes have an out-degree close to 1000.
    \item \textit{Ethererum:}
    More than 90\% of nodes have a degree equal to 0. 
    5\% of the nodes have a degree near 60 and the rest near 120.
    \item \textit{Litecoin:}
    2 regions again, as with in-degree. In and out degree distributions are different in shape.
    In the region with higher jaccard index, 15\% of nodes have a degree between 200 and 1000.  In the other region we have more nodes with zero degree and a percentage 0f 5\% has a degree between 200 and 1000.
    \item \textit{ZCash:}
    Like the other blockchains, most nodes have a 0 out-degree. 12\% if nodes have a degree between 200 and 900.
\end{itemize}


\subsection{Clustering Coefficient distribution}
\begin{itemize}
    \item \textit{Bitcoin:}
    Most nodes have a local clustering coefficient of 0.0.
    A significant percentage around 40\% has a \texttt{cc} between 0.1 and 0.4. 5 to 10\% of nodes have a local \texttt{cc} near 1.0
    \item \textit{BitcoinCash:}
    In BitcoinCash we can't distinguish a general pattern for the distribution of the clustering coefficient.
    \item \textit{DASH:}
    We observe small steps in the \texttt{cc} distribution, around values of 0.1 and 0.3. Most nodes (60\%) have a \texttt{cc} around 0.4.
    \item \textit{Dogecoin:}
    As with the other metrics, Dogecoin has two distinguishable groups of istributions. Most nodes have a \texttt{cc} of 0.8 and 0.95 in the two regions respectively.
    \item \textit{Ethererum:}
    Most nodes in Ethereum have a small \texttt{cc}, less than 0.2. Less than 3\% of the nodes have coefficients greater than 0.3.
    \item \textit{Litecoin:}
    2 regions. The first has a great percentage of nodes with 0.0 \texttt{cc}. Around 20\% of the nodes have a \texttt{cc} near 0.5. The second region has the majority of nodes (70\%) around the same value (0.5).
    \item \textit{ZCash:}
    In ZCash most nodes have either a local \texttt{cc} of 0.0 or 1.0. The rest of the nodes (20\%) have a \texttt{cc} between 0.4 and 1.0. 
\end{itemize}

\subsection{Betweeness Centrality distribution}
\textbf{Graphs are not normalized.}\\
With the exception of DASH, the majority of nodes in all blockchains have betweeness centrality of 0.0.

\begin{itemize}
    \item \textit{Bitcoin:}
    Roughly 10\% of the nodes have a betweeness centrality between 500 and 2000.
    \item \textit{BitcoinCash:}
    Very few nodes (less than 2.5\%) have a centrality near 100. Grater values of centrality are observed in even fewer nodes.
    \item \textit{DASH:}
    DASH nodes have a centrality distributed between 100 and 1000, similar to the distribution of out-degree.
    \item \textit{Dogecoin:}
    Roughy 10\% of the nodes have a centrality near 20 (an order of magnitude less than the out-degree = 200)
    \item \textit{Ethererum:}
    (Focusing on the distributions with higher Jaccard distance - blue hue)
    5\% of nodes between 200 and 2000 (centrality is an order of magnitude greater than out-degree).
    \item \textit{Litecoin:}
    Two distinguishable regions. Both regions rise for betweenes values in the 200 - 1000 range (similar to the out-degree).
    \item \textit{ZCash:}
    The betweeness centrality distributions looks similar to the out-degree distribution. The majority of nodes that have  centrality greater than 0.0, have a \texttt{cc} value near 20 (on order of magnitude less than the out-degree which is between 200 and 900).
\end{itemize}

\subsection{Out degree vs Clustering and Betweeness}
According to Wikipedia:
\textit{"Another important characteristic of scale-free networks is the clustering coefficient distribution, which decreases as the node degree increases. This distribution also follows a power law."}

Figures \ref{fig:btc-other-cc} and  \ref{fig:dash-other-cc}
plot the node degree ($in_{degree} + out_{degree}$) 
against the average clustering coefficient of each degree, for Bitcoin and DASH respectively.

In Bitcoin we can see that the clustering coefficient is higher for low degree nodes but the distribution does not fit a power law.
We can't observe a similar relation in DASH.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/other/btc_dg_cc.png}
  \caption{Degree Vs Average Clustering Coefficient (Bitcoin).
  Line colours correspond to snapshot timestamp.}
  \Description{Bitcoin DegreeVsCC.}
  \label{fig:btc-other-cc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/other/btc_dg_bc.png}
  \caption{Degree Vs Average Betweeness Centrality (Bitcoin).
  Line colours correspond to snapshot timestamp.}
  \Description{Bitcoin DegreeVsBC.}
  \label{fig:btc-other-bc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/other/dash_dg_cc.png}
  \caption{Degree Vs Average Clustering Coefficient (DASH).
  Line colours correspond to snapshot timestamp.}
  \Description{DASH DegreeVsCC.}
  \label{fig:dash-other-cc}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/other/dash_dg_bc.png}
  \caption{Degree Vs Average Betweeness Centrality (DASH).
  Line colours correspond to snapshot timestamp.}
  \Description{DASH DegreeVsBC.}
  \label{fig:dash-other-bc}
\end{figure}
